Efficient and Reliable Hitting-Set Computations for the Implicit Hitting Set Approach

The implicit hitting set (IHS) approach offers a general framework for solving computationally hard combinatorial optimization problems declaratively. IHS iterates between a decision oracle used for extracting sources of inconsistency and an optimizer for computing so-called hitting sets (HSs) over the accumulated sources of inconsistency. While the decision oracle is language-specific, the optimizers is usually instantiated through integer programming. We explore alternative algorithmic techniques for hitting set optimization based on different ways of employing pseudo-Boolean (PB) reasoning as well as stochastic local search. We extensively evaluate the practical feasibility of the alternatives in particular in the context of pseudo-Boolean (0-1 IP) optimization as one of the most recent instantiations of IHS. Highlighting a trade-off between efficiency and reliability, while a commercial IP solver turns out to remain the most effective way to instantiate HS computations, it can cause correctness issues due to numerical instability; in fact, we show that exact HS computations instantiated via PB reasoning can be made competitive with a numerically exact IP solver. Furthermore, the use of PB reasoning as a basis for HS computations allows for obtaining certificates for the correctness of IHS computations, generally applicable to any IHS instantiation in which reasoning in the declarative language at hand can be captured in the PB-based proof format we employ.

==> implementation.tex <==
%!TEX root = ../HittingSetComputationInIHS.tex 
% So that Jeremias IDE plays nice... 


\subsection{Hanneses Notes, to be removed}
To use RoundingSAT as an optimizer we have a parameter to select core-guided or solution-improving search mode for the optimization.
In solution-improving search, there are two variants.
Either solution-improving constraints are added as ``hard constraints'' or as reified constraints
Using ``hard constraints'' is generally faster on individual optimization problems, but has the downside that the optimizer may need to be restarted between IHS iterations.
When reified constraints is used, the optimizer uses the same instantiation of RoundingSAT as a backend, keeping all potentially beneficial learnt information.

In core-guided mode, RoundingSAT is used incrementally, so that on a new IHS iteration the core-guided search continues from where it left on last iteration
(existing reformulation, known LB, and refined objective are kept as they are).
The mplementation also supports restarting the core-guided search, i.e., starting from the original objective again, but we didn't use this option in the experiments: in the default settings, core-guided search never restarts.
The core-guided search is Christoph's implementation.
To be able to use core guided solver incrementally three techniques (hardening, using solution-improving constraints, and cgCoreUpper) were turned off.
(I'm not entirely sure what cgCoreUpper does, based on RoundingSAT help-message, it ``exploits upper bound on cardinality cores'').

Note: in our implementation, objective variables are still hardened in roundingsat-core-guided optimizer, when the hardening happens on global IHS level.
We also use solution-improving constraints in roundingsat-cg optimizer, based on global upper bound for the solution.
(The default option in our implementation is that the (global) solution-improving constraint is used. I'm not sure if we have experiments of it's impact, but sis constraint helps in roundingsat so it probably helps here also)


The solution-improving search we implemented ourselves; RoundingSAT is used only as a decision oracle.
We implemented core-boosting to the sis to improve performance.
In core-boosting, a set of cores is extracted with weight-aware core extraction (one iteration of WCE), OLL-style transformation is applied to them,
and then refined objective is used in solution-improving search.
In addition to extracting cores, core-boosting implementation makes direct use of constraints in the hs-instance (as all the constraints are cores).
(though not all constraints can be directly used in core-boosting, since core-boosting requires that cores imply cost!
For example, if $O= x_1+~x_2$, $x_1+x_2\ge 1$ is a core in a sense that we would seed it, but it couldn't be used in core-boosting, since it doesn't imply cost)
Considering extracted core $C$, $|C|=k$ (number of literals), the core-boosting algorithm first processes all constraints of the hs-instance that have $|C'|<k$ if any of them can be used for core boosting.
The idea is that when processing $C$, if we happen to know a core $D$ that has less literals in it, process $D$ first.


We extended the main IHS solver to support ``exact optimizer'' to support hybrid mode where ``inexact optimizer'' and ``exact optimizer'' are used.
When ``exact optimizer'' is used, lower bound is updated only based on exact optimizer calls.
There are three different options how exact optimizer is used

\begin{enumerate}
\item Every time optimizer claims it has found an optimal solution, and the solution would improve the known LB exact optimizer is invoked and enforced to find optimal solution
\item When the optimizer claims that it has found an optimal solution, and the cost of the solution is UB (the search would terminate), exact optimizer is invoked and enforced to find optimal solution
\item Every time IHS solver (heuristically) decides to find an optimal solution, exact optimizer is invoked (normal optimizer is not invoked). By default, the solver heuristically enforces optimizer to find optimal solution when no cores were found on the iteration, or the LB hasn't changed for $1000$ iterations.
\end{enumerate}

Options 1 and 3 (or similarly options 2 and 3) can be used at the same time (but we do not do this in the experiments).

